Structure Factors of Neutron Matter at Finite Temperature

We compute continuum and infinite volume limit extrapolations of the structure factors of neutron matter at finite temperature and density. Using a lattice formulation of leading-order pionless effective field theory, we compute the momentum dependence of the structure factors at finite temperature and at densities beyond the reach of the virial expansion. The Tan contact parameter is computed and the result agrees with the high momentum tail of the vector structure factor. All errors, statistical and systematic, are controlled for. This calculation is a first step towards a model-independent understanding of the linear response of neutron matter at finite temperature, a realm until now little explored.

==> tuning.tex <==
\section{Tuning The Scattering Length}
Explain in this section how we know that 
\beq
g = \frac{1}{M}\Big(\frac{c_1}{\Delta x} - \frac{1}{4\pi a} \Big)^{-1}~,
\label{eq:coupling-tuning}
\eeq
is the correct tuning procedure. 
